Two-variable logics with some betweenness relations: Expressiveness, satisfiability and membership

We study two extensions of FO2[<], first-order logic interpreted in finite words, in which formulas are restricted to use only two variables. We adjoin to this language two-variable atomic formulas that say, "the letter $a$ appears between positions $x$ and $y$" and "the factor $u$ appears between positions $x$ and $y$". These are, in a sense, the simplest properties that are not expressible using only two variables. We present several logics, both first-order and temporal, that have the same expressive power, and find matching lower and upper bounds for the complexity of satisfiability for each of these formulations. We give effective conditions, in terms of the syntactic monoid of a regular language, for a property to be expressible in these logics. This algebraic analysis allows us to prove, among other things, that our new logics have strictly less expressive power than full first-order logic FO[<]. Our proofs required the development of novel techniques concerning factorizations of words.

==> ksat.tex <==
\section{Temporal logics and satisfiability}\label{sec:tlsat}
\newcommand{\oomit}[1]{}

We denote by $\utl$ temporal logic with two operators $\fut$ and $\past.$  Atomic formulas are propositions
$p\in PV$, a finite set of propositions.  Formulas are built from atomic formulas by applying the boolean operations $\wedge,\vee,$ and $\neg,$ and the modal operators $\gamma\mapsto \fut\gamma,$ $\gamma\mapsto\past\gamma.$

Temporal logics have been interpreted over infinite as well as finite words. Here we confine ourselves only to finite words.
So the propositions $PV$ can be just the alphabet $A$.
We interpret these formulas in marked words. Thus $(w,i)\models a$ if $w(i)=a,$ where $w(i)$ denotes the $i^{th}$ letter of $w.$ Boolean operations have the usual meaning. We define $(w,i)\models \fut\gamma$ if there is some $j>i$ such that $(w,j)\models\gamma,$ and $(w,i)\models\past\gamma$ if there is some $j<i$ with $(w,j)\models\gamma.$

In the setting of verification, it is convenient working with words over a \emph{set} of propositions $\wp(PV)$
as the alphabet, and a boolean formula determining the set which holds at a position $i$.
We also find it convenient to use a set of propositions in Section~\ref{sec:twosat}
where we have to perform reductions between problems.

We can also interpret a formula in ordinary, that is, unmarked words, by defining $w\models\gamma$ to mean $(w,1)\models\gamma.$  Thus temporal formulas, like first-order sentences, define languages in $A^*.$  The temporal logic $\utl$ is known to define exactly the languages definable in $FO^2[<]$ (see \cite{EVW,TW}).

The \emph{size} of a temporal logic formula can be measured as usual,
using the parse tree of the formula, or
using the parse \emph{dag} of the formula, where a subformula
occurs only once.
The latter representation is shorter and is used in the
formula-to-automaton construction \cite{VW}.
The complexity of decision procedures for model checking and
satisfiability do not change (see \cite{DGL}).
For our results, we will use the latter notion of \emph{dag-size}.

\subsection{Betweenness of letters}

We now define new temporal logics by modifying the modal operators $\fut$ and $\past$ with {\it betweenness and threshold constraints}---these are versions of the between relations $\diam{u}(x,y)$ and $(a,k)(x,y)$ that we introduced earlier.   Let $B\subseteq A.$  A threshold constraint is an expression of the form $\#B\sim c,$  where $c\geq 0,$ and $\sim$ is one of the symbols $\{<,\leq,>,\geq,=\}.$ Let  $w\in A^*$ and $1\leq i<j\leq |w|.$ We say that $(w,i,j)$ satisfies the threshold constraint $\#B\sim c$ if
$$|\{k: i<k<j\text{ and }w(k)\in B\}|\sim c.$$
We can combine threshold constraints with boolean operations $\wedge,\vee,\neg.$  We define satisfaction of a boolean combination of threshold constraints in the obvious way--that is, $w(i,j)$ satisfies $g_1\vee g_2$ if and only if $(w,i,j)$ satisfies  $g_1$ or $g_2,$ and likewise for the other boolean operations.

If $g$ is a boolean combination of threshold constraints, then our new operators $\gfut{g}$ and $\gpast{g}$ are defined as follows: $(w,i)\models \gfut{g}\gamma$ if there exists $j>i$ such that $(w,i,j)$ satisfies $g$ and $(w,j)\models\gamma$, $(w,i)\models\gpast{g}\gamma$ if and only if there exists $j<i$ such that $(w,j,i)$ satisfies $g$ and $(w,j)\models\gamma$.

\smallskip
\noindent{\bf Examples.}
\smallskip

\noindent We can express $\fut\gamma$ with threshold constraints as $\gfut{\#\emptyset=0}\gamma.$

\smallskip

\noindent We use $\nextt$ to denote the `next' operator:  $(w,i)\models \nextt\gamma$ if and only if $(w,i+1)\models\gamma.$ We can express this with threshold constraints by $\gfut{\#A=0}\gamma.$

\smallskip

\noindent We can define the language $(ab)^+$ over the alphabet $\{a,b\}$ as the conjunction of several subformulas: $a\wedge \nextt b$ says that the first letter is $a$ and the second $b$.  $\neg \fut (a\wedge \nextt  a)$ says that no  occurrence of $a$ after the first letter is immediately followed by another $a$, and similarly we can say that no occurrence of $b$ is followed immediately by another $b$. The formula $\fut(b\wedge\neg\nextt (a\vee b))$ says that the last letter is $b$.

\smallskip



We denote by  \bthtl\/ temporal logic with these modified operators $\gfut{g}$ and $\gpast{g},$ where $g$ is a boolean combination of threshold constraints.
We also define several fragments of  \bthtl.
In \thtl\/ we further restrict guards $g$ to be atomic, rather than boolean combinations.
In \invtl\/ we restrict to constraints of the form $\#B=0$ -- we call these {\it invariance constraints} since they assert invariance of absence of letters of $B$ in parts of words.
In \binvtl\/ we allow boolean combinations of such invariance constraints.


\smallskip
\noindent{\bf Example.}
\smallskip
It is useful to have boolean combinations of threshold constraints.
The language $STAIR_k$ given in Section \ref{sec:twotwo} can be defined by
$\fut (\gfut{\#a=k \land \#b=0} ~true)$.



\begin{thm}~\label{thm.tlequivalence} The logics \thtl, \bthtl, \invtl, \binvtl,
\fotwothr\/ and \fotwobet\/ all define the same family of languages.
\end{thm}


\subsubsection{Proof of Theorem~\ref{thm.tlequivalence}}

In terms of syntactic classes, we obviously have
$$\invtl\subseteq\binvtl\subseteq\bthtl,$$
and
$$\invtl\subseteq\thtl\subseteq\bthtl.$$

We show that $\bthtl\subseteq\invtl$ using a chain of inclusions
passing through the two-variable logics.
In performing these translations, we will only discuss the future modalities,
since the past modalities can be treated the same way.

We can directly translate any formula in \bthtl\/ into an equivalent formula of \fotwothr\/
with a single free variable $x$:  A formula $\gfut{g}\psi$,
where $g$ is a boolean combination of threshold constraints,
is replaced by a quantified formula $\exists y (y>x \wedge \alpha\wedge \beta(y))$,
where $\alpha$ is a boolean combination of formulas $(a,k)(x,y)$ and $\beta$ is the translation of $\psi$.

We know from Theorem~\ref{thm.invequalsthr} that any formula of \fotwothr\/ can in turn be translated
into an equivalent formula of \fotwobet. Furthermore, \fotwobet\/ is  equivalent to \binvtl:
A simple game argument shows that equivalence of marked words with respect to \binvtl\/ formulas
of modal depth $k$ is precisely the relation $\equiv_k$ of equivalence with respect to
\fotwobet\/ formulas with quantifier depth $k$.

So it remains to show that $\binvtl\subseteq \invtl$:
We do this by translating $\gfut{g}\phi$,
where $g$ is a boolean combination of constraints of the form $\#B=0$,
into a formula that uses only single constraints of this form.

We can rewrite the boolean combination as the disjunction of conjunctions of constraints
of the form $\#\{a\}=0$ and $\#\{a\}>0$.
Since, easily, $\gfut{g_1\vee g_2}\gamma$ is equivalent to $\gfut{g_1}\gamma \vee\gfut{g_2}\gamma$,
we need only treat the case where $g$ is a conjunction of such constraints.
We  illustrate the  general procedure  for translating such conjunctions with an example.
Suppose $A$ includes the letters $a,b,c$.
How do we express $\gfut{g}\gamma$, where $g$ is $(\#\{a\}=0)\wedge(\#\{b\}>0)\wedge(\#\{c\}>0)$?
The letters $b$ and $c$ must appear in the interval between the current position
and the position where $\gamma$ holds.  Suppose that $b$ appears before $c$ does.  We write this as
$$\gfut{\#\{a,b,c\}=0}(b\wedge\gfut{\#\{a,c\}=0}(c\wedge\gfut{\#\{a\}=0}\gamma)).$$
We take the disjunction of this with the same formula in which the roles of $b$ and $c$ are reversed.


\subsection{Betweenness of factors}

We denote by \bthfactl\/ temporal logic with these modified operators $\gfut{g}$ and $\gpast{g},$ where $g$ is a boolean combination of threshold factor constraints.
We also define several fragments of \bthfactl:  For example, \bfactl\/ has the modalities
$\gfut{R}\gamma$ and $\gpast{R}\gamma$ where $R$ is a boolean combination
of \emph{requirements on occurrences of factors}.
Since disjunctions can be pulled out,
we write the conjunctive requirements as a finite set of positive and negative
factors. Logic \factl\/ is a further restricted version where there are no positive requirements and a single  negative requirement is permitted, i.e. $R$ has the form
$\{\neg v\}$.

\smallskip

\noindent{\it Notation.}
For convenience,
for $u = a_1 a_2\dots a_n$, we will abbreviate by $st(u)$ the \ltl\/ formula
$a_1 \land \nextt(a_2 \land (\dots \land \nextt a_n))$ and by
$end(u)$ the formula $a_n \land \prev(a_{n-1} \land (\dots \land \prev a_1))$.
Also, for $u=\epsilon$ (empty string) define $st(u)=end(u)=true$.

\smallskip
\noindent{\bf Examples.}
\smallskip

The formula $\henceforth(st(bb) \limplies \past(end(aa)))$ specifies that
there is no factor $bb$ which is not preceded by an $aa$.

\smallskip

$\henceforth(st(bb) \land \past(end(bb)) \limplies \gpast{aa}(end(bb))))$ says
that between any two occurrences of $bb$ there must be an $aa$.

\medskip

Formally, we have $(w,i)\models \gfut{R}\gamma$ if for some $j>i$, $(w,j)\models \gamma$
and for every positive factor $u \in R$ there is an occurrence of factor $u$
between, that is, for some $i < k < k+|u|-1 < j$, $(w,k)\models st(u)$,
and for every negative factor $\lnot v \in R$ there is no occurrence of
factor $v$ between,
that is, for all $i < k < k+|v|-1 < j$, $(w,k)\not\models st(v)$.
%A positive occurrence of a factor $u$ is definable in temporal logic \ltl\/
%as $\fut(u \land \nextt^{|u|}\fut\gamma)$.
\bigskip

\begin{thm}~\label{thm.factlequivalence}
The logics \bthfactl, \bfactl, \factl, \fotwothrfac\/ and \fotwobetfac\/ all define the same family of languages.
\end{thm}

As in the proof of Theorem \ref{thm.tlequivalence}, the key question is how to translate
\bfactl\/ into \factl. All other reductions are straightfoward extensions (substituting factors in place of letters) of those given in the previous proof. Hence we omit repeating these.
For showing $\bfactl \subseteq \factl$, We consider the modality
$\gfut{\{u_1,\ldots,u_p, \neg v_1, \ldots, \neg v_r\} } \gamma$  and construct an equivalent
formula using only the modality of the form $\gfut{\{\neg v\}} \gamma$.

\begin{lem} \label{lem:singlepair}
$\gfut{\{u_1,\ldots,u_p, \neg v_1, \ldots, \neg v_r\} } \gamma \quad \equiv \quad
 \bigwedge_{1 \leq i \leq p} \bigwedge_{1 \leq j \leq r} \gfut{\{u_i,\neg v_j\}} \gamma$.
 The dag-size of the right hand formula is polynomial in the size of the left hand formula.
\end{lem}
\begin{proof}
First note that
\[
\gfut{\{u_1,\ldots,u_p, \neg v_1, \ldots, \neg v_r\} } \gamma \quad \equiv \quad
 \bigwedge_{1 \leq i \leq p} \gfut{\{ u_i, \neg v_1, \ldots, \neg v_r\} } \gamma
\]
The forward direction is clear. For the converse, let $k$ be the position where the right hand
conjunction holds. Let $x_i > k$ such that
$(w,x_i)\models \gamma$ witnessing $(w,k)\models \gfut{\{ u_i, \neg v_1, \ldots, \neg v_r\} } \gamma$.
Consider $x=max\{x_i\}$. Then, $(w,x)\models \gamma$ witnessing the left hand formula.

Also,
\[
\gfut{\{ u, \neg v_1, \ldots, \neg v_r\} } \gamma \quad \equiv \quad
 \bigwedge_{1 \leq j \leq r} \gfut{\{u,\neg v_i\}} \gamma
\]
The forward direction is clear. For the converse, let $k$ be the position where the right hand
conjunction holds. Let $x_i > k$ s.t.
$(w,x_j)\models \gamma$ witnessing $(w,k)\models \gfut{\{ u, \neg v_j\}}$.
Consider $x=min\{x_i\}$. Then, $(w,x)\models \gamma$ witnessing the left hand formula.

The result follows by combining the two steps. It is also clear that resulting formula has $p.r$ conjuncts of constant size which each use $\gamma$ as subformula. Hence, the dag-size of the conjunction is polynomial
in the size of the left hand formula.
\end{proof}

\input{fig-overlap}

Because of above lemma we only need to consider formulas with modalities of the form
$\gfut{\{u,\neg v\}} \gamma$.
We reduce them to a formula only using the modalities of the form
$\gfut{\{\neg v\}} \gamma$ which we abbreviate as $\gfut{\neg v}\gamma$.

We have to consider several cases which are illustrated in Figure~\ref{fig:overlap}.
Notice that, from the semantics, $(w,x)\models \gfut{\{u,\neg v\}} \gamma$ {\bf iff} for given $w,x$ there exist
$s,e,y$ such that $x < s < e < y$ and {\bf (1)} $w[s,e]=u$, {\bf (2)} $(w,y)\models \gamma$, and {\bf (3)} $v$ is not a factor of $w[x+1,y-1]$.
Then, the above condition (3) that  $v$ is not a factor of $w[x+1,y-1]$ is equivalent to the conjunction of conditions: $v$ is not a factor of any of {\bf (3a)}  $w[x+1,s-1]$, {\bf (3b)} $w[s,e]$, {\bf (3c)} $w[e+1,y-1]$,  {\bf (3d')} $v$ does not overlap $u$ at $s$, {\bf (3e')}  $v$ does not overlap $e$
at $b$, and {\bf (3f')} $v$ does not overlap $u$ at both $s$ and $e$, that is, $u$ is not a factor wholly inside $v$.

Overlaps of the form (3d'), (3e') and (3f') will be called pre-overlaps, post-overlaps and sub-overlaps, respectively.

If $u=u_1 \cdot v \cdot u_2$, then condition 3(b) is violated, and  trivially
$\gfut{\{u,\neg v\}} \gamma \equiv \false$.  In the rest of the section, we assume that $v$ is not a factor of $u$, and hence condition (3b) is always satisfied.

Note that there can be several occurrences of $u$ after $x$ and several occurrences of
$\gamma$ after the end of $u$.

\begin{lem} \label{lem:earlyu} Let $w$ and $x<s<e<y$ satisfy conditions (1),(2),(3a-3c,3d'-3f'),
and let  $w$ and $x<s'<e'<y'$ satisfy conditions (1) and (2). If $s'<s \land e'<e \land y' <y$ then
 $w$ and $x<s'<e'<y'$ also satisfy conditions (3a-3c,3d'-3f').
\end{lem}

\begin{proof}
Consider the first point where $\gamma$ holds
such that there is an occurrence of $u$ between $x$ and this point. Clearly this is sufficient
from the semantics of the modality. Without loss of generality we can call this point $y$.
Fix this point as $y$.
Observe from the figure that if, instead of the occurrence of $u$ from $s$ to $e$,
one considers a different occurrence of $u$ from $s'$ to $e'$,
any occurrences of $v$ will shift between the categories (3a-3c,3d'-3f').
However any occurrence of $v$ in the categories (3g-3h) continues to be
in the same category for both occurrences of $u$. Hence the allowed and disallowed
categories continue to be the same, and in order to verify the semantics of
the formula we can use any occurrence of $u$.
\end{proof}

\oomit{
First consider the following formula $\beta_1$ which captures conditions (1),(2),(3a), and (3c).
\[
    \gfut{\neg v} ~[ st(u) ~\land~ (\nextt^{(|u|-1)} (\gfut{\neg v} \gamma))]
\]
Note that subformula $st(u)$ is evaluated at position $s$, and subformula $\gfut{\neg v} \gamma$ is evaluated as position $e$. Subformula $\gamma$ is evaluated at position $y$.
\medskip
}


Given words $u$ and $v$, define  $U_1,V_1,U_2,V_2 \subseteq A^*$, where $U_1,U_2$ contain some prefixes of $v$ and  $V_1,V_2$ contain some suffixes of $v$,  as follows:
\begin{itemize}
\item  Let $U_1=\{ v_1 ~\mid~ v=v_1u_1 ~\mbox{and}~ u=u_1u_2 ~\mbox{with}~ u_1,u_2,v_1 \neq \epsilon\}$. ((3d) is violated). $U_1$ give all possible pre-overlaps.
\item Let  $V_1= \{ v_2 ~\mid~ u=u_1u_2 ~\mbox{and}~ v=u_1v_2 ~\mbox{with}~ u_1,u_2,v_2 \neq \epsilon\}$. ((3e) is violated). $V_1$ gives all possible post-overlaps.
\item If $v = v_1 \cdot u \cdot v_2$ with $v_1 \neq \epsilon \lor v_2 \neq \epsilon$ we have sub-overlap. ((3f) is violated). There can be several such $(v_1,v_2)$ pairs.
Using Lemma~\ref{lem:earlyu} it is sufficient to consider the earliest occurrence of $u$,
so we let $U_2=\{v_1\}$ and $V_2=\{v_2\}$ where $v_1,v_2$ are obtained by the factorization of $v$
which makes $v_1$ the shortest. This coincides with the earliest occurrence of $u$, see the example below.
If no such pair $(v_1,v_2)$ exists, let $U_2=V_2=\emptyset$.
Thus, $U_2,V_2$ are either both singleton sets or both are empty.
\end{itemize}

\medskip

\noindent \textbf{Examples.}
For $u=aaa$ and $v=bbb$, trivially, $U_1=V_1=U_2=V_2=\emptyset$ since there are no overlaps.
\smallskip

For $u=ababbb$ and $v=bbabab$, because of pre-overlaps
$(u=abab \cdot bb,v=bb \cdot abab)$ and $(u=ab \cdot ab bb,v=bbab \cdot ab)$, we get $U_1=\{bb,bbab\}$. Note that which of these overlaps will
apply will depend of word $w$. If $w=bbabababbb$ then $U_1$ element $bbab$ will
characterise pre-overlap whereas
if $w=bbababbb$ then $U_1$ element $bb$ will characterize the pre-overlap.
Also, due to post-overlap
$(u=abab \cdot bb,v=bb \cdot abab)$ we have $V_1= \{ abab \}$. Since,
$u$ is not subword of $v$, we have $U_2=V_2=\emptyset$.
\smallskip

For $u=aa$ and $v=aaaabbaaaa$, we have several possible overlaps. The only pre-overlap is  $(v=aaaabbaaa \cdot a,u=a \cdot a)$. Sub-overlaps are  $v=aaaabbaa \cdot aa \cdot$, $aaaabba \cdot aa \cdot a$,
$aaaabb \cdot aa \cdot aa$, $aa \cdot aa \cdot bb aa aa$, $ a \cdot aa \cdot abbaaaa$, $\cdot aa \cdot aa bb aaaa$.
We have one post-overlap $(v=a \cdot aaabbaaaa,u= a \cdot a)$. Hence, we
get $U_1=\{ aaaabbaaa\}$, $V_1=\{aaabbaaaa\}$. It is sufficient to consider the canonical sub-overlap $\cdot aa \cdot aabbaaaa$ giving $U_2=\{ \epsilon \}$ and $V_2=\{ aabbaaaa\}$.
\qed
\medskip


Observe that we can rephrase conditions (3d'-3f') to equivalent conditions (3d-3f) as follows.
\begin{itemize}
 \item (3d) for all $v' \in U_1$ we have $v'$ is not a suffix of $w[x+1,s-1]$.
 \item (3e) for all $v' \in V_1$ we have $v'$ is not a prefix of $w[e+1,y-1]$.
 \item (3f) Since $U_2=V_2 = \emptyset$ or $U_2=\{v_1'\}, V_2=\{v_2'\}$, (3f)
 states that $U_2= \emptyset$, or, $v_1'$ is suffix of $w[x+1,s-1]$ implies $v_2'$ is not a prefix of $w[e+1,y-1]$.
\end{itemize}
Thus, we have:
\begin{lem} \label{lem:formcond}
 $w,x \models \gfut{\{u,\neg v\}} \gamma$ {\bf iff} for given $w,x$ there exist $s,e,y$ s.t.
 $x<s<e<y$ and conditions (1),(2),(3a-3f) are satisfied.
\end{lem}
We now define  $\beta \in \factl$ to enforce conditions (1),(2), (3a-3f). Clearly, this will give
us a formula $\beta$ equivalent to $\gfut{\{u,\neg v\}} \gamma$.

\bigskip

\noindent For $U,V \subseteq A^+$, define
\begin{quote}
 $Prec(U) = \bigvee_{(v' \in U)} ~\prev end(v')$  \\
 $Prec(U,i) = \bigvee_{(v' \in U, |v'|<i)}  ~\prev end(v')$ \\
 $Follow(V) = \bigvee_{(v' \in V)} ~ \nextt st(v')$ \\
 $Follow(V,i) = \bigvee_{(v' \in V, |v'|<i)} \nextt st(v')$ \\
 Note that if $U,V$ are $\emptyset$, then all of these vacuously evaluate to $false$.
\end{quote}
Then,  $(w,s)\models \neg Prec(U)$ states that no $v' \in U$ ends at $s-1$  in $w$.
Moreover, $(w,s)\models \neg Prec(U,i)$ states that no $v' \in U$ of length shorter than $i$ ends at $s-1$.
Formulae $\neg Prec(U)$ and $\neg Prec(U,i)$ will be used to enforce condition (3d). Similarly, formulae
$\neg Follow(V)$ and $\neg Follow(U,i)$ will be used to enforce condition (3e).

\medskip

For given $u,v$, let $U_1,V_1,U_2,V_2$, as well as predicates
$Prec(\cdot), Follow(\cdot)$ on them, be syntactically determined as defined above.
These predicates have to be applied at different points.
We define a subsidiary formula $\delta(V)$ below with a parameter
$V \subseteq \mathit{proper\_prefixes}(v)$ to check the requirements
remaining at the end of an occurrence of $u$. Let $m= max\{|v'| ~\mid~ v' \in V\}$.
\[
\delta(V) = [ (\gfut{\neg v} ~\gamma) ~~\land ~~\neg Follow(V)]
    \lor ~~\bigvee_{i=1}^m ~  [ \neg Follow(V,i) ~~\land~~ (\nextt^i \gamma)]
\]
%\begin{array}{l}
%    \phantom{  \lor ~~ } [ (\gfut{\neg v} ~\gamma) ~~\land ~~\neg Follow(V)] \\
%    \lor ~~\bigvee_{i=1}^m ~
%    [ \neg Follow(V,i) ~~\land~~ (\nextt^i \gamma)]
%\end{array}

\begin{lem} \label{lem:deltacond}
 For any given $V \subseteq \mathit{proper\_prefixes}(v)$, we have
 $w,e \models \delta(V)$ {\bf iff} for given $w,e$ there exists $y$ s.t. $e < y$ and conditions
 (2), (3c)  and there are no post-requirements, by which we mean
 the condition (n1): for all $v' \in V$, $v'$ is not a prefix of $w[e+1,y-1]$.
\end{lem}
\begin{proof}
(LHS implies RHS) Let $w,e \models \delta(V)$. \\
Case 1: $w,e \models (F_{\neg v} \gamma) \land \neg Follow(V)$. Then by the semantics of modality $F_{\neg v} \gamma$, conditions (2) and (3c) are satisfied. Also, the conjunct $\neg Follow(V)$ ensures that any $v' \in V$ is not a prefix of $w[e+1,|w|-1]$ and hence also of $w[e+1,y-1]$. Thus, (n1) is satisfied. \\
Case2 : $w,e \models \neg Follow(V,i) ~~\land~~ (\nextt^i \gamma)$ for some $1 \leq i \leq m$. Note that $m<|v|$.
Taking $y=e+i$ we get that (2) is satisfied. Moreover, (3c) is satisfied as interval $(e,y)$ of length $i$ is
too small to accommodate $v$. Finally, conjunct $\neg Follow(V,i)$ ensures (n1).
\medskip

\noindent (RHS implies LHS). Let $w,e,y$ s.t. $e<y$ and (2),(3c)  and (n1) are satisfied.\\
Case 1:   $y-e > m$. Then,  $F_{\neg v} \gamma$ follows from (2) and (3c), by the semantics.
By (n1), every $v' \in V$ is not prefix of $w[e+1,y-1]$. But as $y-e>m$ and $|v'| \leq m$, we have any $v'$ starting at $e+1$ must end before position $y$. Hence, $w,e \models \neg Follow(V)$. Thus, $w,e$ satisfies the first disjunct of $\delta(V)$.\\
Case 2: $y-e \leq m$. In this case, $v$  cannot occur between $e+1$ and $y-1$ as $|v| > m$. Let $i=y-e$.
Then by (2) we have $w,e+i \models \gamma$ giving $w,e \models X^i \gamma$. Also, by (n1), for all
$v' \in V$ with $|v'| <i$ we have $v'$ is not a prefix of $[e+1,y-1]$. Hence, $w,e \models \neg Follow(V,i)$.
Thus, $w,e$ satisfies the second disjunct of $\delta(V)$.
\end{proof}
\medskip

\noindent We now define $\beta$.
Let $k = max\{|v'| ~\mid~ v' \in U_1 \cup U_2\}$.
Then, $\beta(U_1,V_1,U_2,V_2)$ is given by
\[
\begin{array}{l}
  \phantom{\lor ~~}    \gfut{\neg v} ~[st(u) ~\land~ \neg Prec(U_1) \land
	[ \quad [\neg Prec(U_2) ~\land~ \nextt^{(|u|-1)} (\delta(V_1))] \\
	     \hspace*{5.2cm} \lor [~ Prec(U_2) ~\land~
                       \nextt^{(|u|-1)} (\delta(V_1 \cup V_2))]~~]~~] \\
  \lor ~~ \bigvee_{i=1}^{k} ~\nextt^i
	    [st(u) ~\land~ \neg Prec(U_1,i)\land [ \quad [(\neg Prec(U_2,i)) ~\land~ \nextt^{(|u|-1)} (\delta(V_1))]  \\
               \hspace*{6.2cm} \lor~ [Prec(U_2,i) ~\land~
                 ~\nextt^{(|u|-1)} (\delta(V_1 \cup V_2)) ]~~]~
            ]
   \end{array}
\]
%The formula $w,x \models \beta(U_1,V_1,U_2,V_2)$ enforces conditions (1),(3a),(3d) in addition to invoking $\delta$.
\begin{lem} \label{lem:nfacred}
 $w,x \models \beta$ {\bf iff} for given $w,x$ there exist $s,e$ such that  $x<s<e$ satisfying
 conditions (1),(3a),(3d) and the following implication:

\begin{tabular}{l}
(n2) if $U_2=\{v_1\}$ and $v_1$ is not suffix of $w[x+1,s-1]$,
then $w,e \models \delta(V_1 \cup V_2)$,\\
\hspace{1cm} else $w,e \models \delta(V_1)$.
\end{tabular}
\end{lem}
\begin{proof}
There are two cases, $U_2=V_2=\emptyset$, and $U_2=\{v_1\}, V_2=\{v_2\}$.
We consider the more complex second case.
(The first case is similar to a subcase of the second one and omitted.)
\medskip

(LHS implies RHS) Let $w,x \models \beta$. Notice that $\beta$ has two disjuncts. \\
Case 1: $w,x$ satisfies first disjunct. By subformula $w,x \models F_{\neg v} [st(u)]$,
condition (1) and (3a) are satisfied. Further subformula $\neg Prec(U_1)]$ ensures that every $v' \in U_1$ does not end at $s-1$ and hence it cannot be a suffix of $w[x+1,s=1]$. Hence (3d) is satisfied. The remaining subformula (consisting of two aub-disjuncts) will imply (n2). In case the first sub-disjunct holds, we have, $w,s \models \neg Prec(U_2)$ which implies $v_1$ is not a suffix of $w[x+1,s-1]$. Then, the formula asserts $\delta(V_1)$, hence satisfying (n2). If the second disjunct holds,we have two possibilities. Either  $v_1$ is a prefix of $w[x+1,s-1]$ and as the formula asserts $\delta(V_1 \cup V_2)$ condition (n2) holds. Otherwise, $v_1$ is not a prefix of $w[x+1,s-1]$ (although $Prec(U_2)$ holds).
The formula asserts $\delta(V_1 \cup V_2)$ which implies $\delta(V_1)$ and hence (n2) holds.
We note that this case overlaps with case 2, below, where weaker formula $\delta(V_1)$ is asserted. \\
Case 2: $w,x$ satisfies second disjunct. Then for some $1 \leq i \leq k$ we have
$w,x \models X^i st(u)$, which by taking $s=x+i$, gives (1). Also $i \leq k < |v|$ giving (3a) as interval $x+1,s-1$ is too small to contain $v$. Finally, notice that  $v'$ is suffix of $w[x+1,s-1]$ iff $w,s \models Prec(U_2,i)$. Hence, the subformula with two sub-disjuncts is equivalent to (n2).
\medskip


(RHS implies LHS) For given $w,x$ there exist $s,e$ such that $x<s<e$ and (1),(3a),(3d) and (n2) are satisfied. We consider two cases $s-x > k$ and $s-x \leq k$.
\\
(Case 1: $s-x > k$) By (1) and (3a), we have $w,x \models F_{\neg v} st(u)$. Also, (3d) states that for all $v' \in U_1$, we have $v'$ is not a suffix of $w[x+1,s-1]$. But, as
$|v'| \leq k$ and $s-x > k$ we have $v'$ does end at $s+1$. Hence, $w,s \models \neg Prec(U_1)$. By similar reasoning $v_1$ is a suffix of $w[x+1,s-1]$ iff $w,s \models Prec(U_2)$. Then, (n2) is equivalent to the subformula with two disjuncts. \\
(Case 2: $s-x \leq k$). Let $i=s-x$. Then $1 \leq i \leq k$. By (1) we have $w,x \models X^i st(u)$. By (3e), for all $v' \in U_1$ with $|v'| < i$, we have $v'$ does not end at $s-1$,
giving $w,s \models \neg Prec(U_1,i)$. Similarly, $v_1$ is not a suffix of $w[x+1,s-1]$ iff
$v_1$ does not end at $s-1$ iff $w,s \models \neg Prec(U_2,i)$. Hence, (n2) is equivalent
to subformula with two disjuncts.

This completes the proof of the lemma. It is easy to see that the dag-size of $\beta$,
with the $\delta$ occurrences substituted out,
is polynomial in the size of $\gfut{\{u,\neg v\}} \gamma$.
\end{proof}

By Lemma \ref{lem:deltacond}, the post-requirement holds iff
the conditions (2),(3c),(3e) and (3f) hold.
Hence we have $w,x \models \gfut{\{ u, \neg v\}}\gamma$ iff $w,x \models \beta$.
The result that $\bfactl \subseteq \factl$ follows from this
by first applying Lemma \ref{lem:singlepair}.
This completes the proof of Theorem \ref{thm.factlequivalence}.

\bigskip

Now we give a reduction from \factl\/ to \ltl.
\begin{lem}\label{lem.toltl}
For $\gfut{\neg v} \gamma$ we have an equivalent \ltl\/ formula:
\[
 (\bigvee_{i=1}^{|v|-1} \nextt^i \gamma)  ~~\lor~~ ( (\neg end(v)) \until \gamma).
\]
\end{lem}
The proof follows from the semantics. Note that the dag-size of the \ltl\/ formula is polynomial in the size of $\gfut{\neg v} \gamma$. \qed



\subsection{Complexity of satisfiability}\label{KamalParitosh}

Given a formula in one of these logics, what is the computational complexity of determining whether it has a model, that is, whether the language it defines is empty or not?  This is the {\it satisfiability problem}  for the logic.  To determine this, we require some way to measure the size of the input formula.  For formulas containing threshold constraints, we code the threshold value in binary, so that mention of a threshold constant $c$ contributes $\lceil\log_2 c\rceil$ to the size of the formula. Mention of a subalphabet $B$ contributes $|B|$ to the size of the formula.
Our results below hold for bounded and unbounded alphabets,
which may be explicitly specified or symbolically specified by propositions.
Recall that we use the dag-size, that is, the input formula
is represented as a dag (see \cite{DGL}).

\begin{thm}\label{thm.utlsat}
The satisfiability problems for the temporal logics $\bfactl,\binvtl$ (with boolean combination of invariance constraints)
are \pspace-complete.
The satisfiability problems for $\bthfactl,\bthtl$ (with boolean combination of threshold constraints)
are \expspace-complete.
\end{thm}

We think that providing such factor requirements in temporal
logic, using our simple notation, improves convenience without sacrificing
complexity of satisfiability. Threshold requirements provide greater
succinctness, but that comes with a computational cost.

\begin{proof}
Satisfiability of \invtl\/ is \pspace-hard \cite{SC} since it includes
\ltlunsuc.
We observe that \binvtl\/ can be translated into \ltlbin\/ in polynomial time,
hence its satisfiability is \pspace-complete \cite{SC}.
Using a threshold constant $2^n$, written in binary in the formula with size $n$,
the  $2^n$-iterated Next operator $X^{(2^n)}$ can be expressed in \thtl,
so we obtain that its satisfiability is \expspace-hard \cite{AH}.
By an exponential translation of \bthtl\/ into \binvtl,
(the proof of Theorem~\ref{thm.invequalsthr} shows that such translation exists), or alternately by a polynomial
translation into \cltlbin\/ \cite{LMP},
its satisfiability is \expspace-complete.
Analogously we can translate from \bthfactl\/ into \bfactl
(for which we have to rely on Theorem~\ref{thm.invequalsthrfac}).

Giving the upper bound for the factor logic \bfactl\/ takes more work,
but nearly all of it has been done in Theorem~\ref{thm.factlequivalence},
using which we translate to an \factl\/ formula with
polynomially larger dag-size, which only uses singleton negative
requirements. By Lemma~\ref{lem.toltl} this translation can be continued
into an \ltl\/ formula
which uses the binary \emph{until} operation (but no nested \emph{until}'s),
and the decision procedure for \ltl\/ \cite{SC} completes the proof.
\end{proof}

\subsection{Satisfiability of two-variable logics}\label{sec:twosat}

\begin{thm}
\label{thm.fo2sat}
Satisfiability of the two-variable logics
\fotwobet, \fotwobetfac, \fotwothr\/ and \fotwothrfac\/ is \expspace-complete.
\end{thm}

We begin by reducing the \emph{exponential Corridor Tiling problem}
to satisfiability of \fotwobet.
It is well known that this problem is \expspace-complete \cite{Furer}.
An instance $M$ of the problem is given by $(T,H,V,s,f,n)$
where $T$ is a finite set of tile types with $s,f \in T$,
the horizontal and vertical tiling relations
$H, V \subseteq T \times T$, and $n$ is a natural number.
A solution of the $2^n$ sized corridor tiling problem is
a natural number $m$ and map $\pi$ from
the grid of points $\{ (i,j) ~\mid~ 0 \leq i \leq 2^n,~0 \leq j < m\}$
to $T$ such that: \\
$\pi(0,0)=s$, $\pi(2^n-1,m-1)=f$ and for all $i$, $j$ on the grid, \\
$(\pi(i,j),\pi(i,j+1)) \in V$ and $(\pi(i,j),\pi(i+1,j)) \in H$.

\begin{lem}
\label{lem.tiling}
Satisfiability of the two-variable logic \fotwobet\/ is \expspace-hard.
\end{lem}
\begin{proof}
Given an instance $M$ as above of a Corridor Tiling problem,
we encode it as a sentence  $\phi(M)$ of size $poly(n)$ with a
modulo $2^n$ counter $C(x)$ encoded serially with $n+1$ letters.
As we already saw in the examples in Section \ref{sec:examples},
the counter could be laid out using successive $n+1$ letter substrings
to represent $n$ bits (over a subalphabet of size $2$) preceded by a marker.
The marker now represents a tile and a colour from $red$, $blue$ and $green$
(requiring subalphabet size $3|T|$).
Thus the $2^{n} \times m$ tiling is represented by a word of length
$m(n+1)2^n$ over an alphabet of size $3|T|+2$.
The claim is that $M$ has a solution iff $\phi(M)$ is satisfiable.

The sentence  $\phi(M) \in \fotwobet$ is a conjunction of
the following properties.
The key idea is to cyclically use monadic predicates
$red(x), green(x), blue(x)$ for assigning colours to rows.

\begin{itemize}
\item
Each marker position has exactly one tile and one colour.
\item
The starting tile is $s$, the initial colour is $red$,
the initial counter bits read $0^n$, the last tile is $f$.
\item
Tile colour remains same in a row and it cycles in order
$red,green,blue$ on row change.
\item
The counter increments modulo $2^n$ in consecutive positions.
\item
For horizontal compatibility we check:\\
$
\begin{array}{l}
\forall x \forall y(mark(x) \land mark(y) \land \neg mark(x,y)
\limplies \\
 \hspace*{1cm} \orover_{(t_1,t_2) \in H} ~ t_1(x) \land t_2(y))
\end{array}
$.
\item
For vertical compatibility, %This is the main part of the formula.
we check that $x,y$ are in adjacent rows by invariance of lack of one colour.
We check that $x$ and $y$ are in the same column by checking that
the counter value (which encodes column number) is the same:
\[ \forall x \forall y ( (x < y) \land
(\neg red(x,y) \lor \neg blue(x,y) \lor \neg green(x,y)) \land EQ(x,y) \limplies
\orover_{(t_1,t_2) \in V} ~ t_1(x) \land t_2(y)).
\]
\end{itemize}

It is easy to see that we can effectively translate an instance $M$ of
the exponential corridor tiling problem into $\phi(M)$ in time
polynomial in $n$. The translation preserves satisfiability.
Hence, by reduction, satisfiability of $\fotwobet$ over bounded
as well as unbounded alphabets is $\expspace$-hard.
\end{proof}

\begin{lem}
\label{lem.reduction}
There are satisfiability-preserving polynomial time reductions from
the logic \fotwothr\/ to the logic \fotwobet, and from
the logic \fotwothrfac\/ to the logic \fotwobetfac.
\end{lem}
\begin{proof}
We give a polytime reduction from \fotwothr\/ to  \fotwobet\/
which preserves satisfiability. The same idea works for the reduction
from \fotwothrfac\/ to \fotwobetfac.
We consider in the extended syntax
a threshold constraint  $\#a(x,y)=k$ where $a$ is a letter or a proposition and
$k$ is a natural number.
The key idea of the reduction is illustrated by the following example.

For each threshold constraint $g$ of the form $\#a(x,y)=2^r$,
we specify a \emph{global} modulo $2^r$ counter $C_g$
using monadic predicates
$p_1(x), \ldots, p_r(x)$ whose truth yield an $r$-bit vector denoting  the value of the counter at position $x$.
(This requires a symbolic alphabet
where several such predicates may be true at the same position.)
By ``global'' we mean that the counter $C_g$ has value $0$
at the beginning of the word and it increments whenever $a(x)$ is true.
This is achieved using the formula:
\[
\forall x,y (\suc(x,y) \limplies (a(x) \limplies INC_g(x,y)) \land
 (\neg a(x) \limplies EQ_g(x,y)))
\]
Here, the formulas $EQ_g(x,y)$ and $INC_g(x,y)$ are similar to those of the serial counter example in Section \ref{sec:examples}.
Also, we have three colour predicates $red_g(x)$, $blue_g(x)$ and $green_g(x)$
where the colour at the beginning of the word is $red_g$,
and we change the colour cyclically each time the counter $C_g$
resets to zero by overflowing.
As in the proof of Lemma~\ref{lem.tiling},
invariance of lack of one colour and the fact that $x,y$ have different colours
ensures that the counter overflows at most once.
We replace the constraint $g$
of the form $\#a(x,y)=2^r$ by an equisatisfiable formula:
\[
\begin{array}{l}
x<y \land EQ_g(x,y) \land \#a(x,y) > 0 \land\\
(\neg red_g(x,y) \lor \neg blue_g(x,y) \lor \neg green_g(x,y))
\end{array}
\]
More generally, we define a polynomial sized quantifier free formula
$INC_{g,c}(x,y)$ for any given constant $c$ with $2^{r-1} <c \leq 2^r$ using
propositions $p_1, \ldots, p_r$ and three colour predicates.
The formula asserts that $\#a(x,y)+ c = 2^r$.
Using this we can encode the constraint $\#a(x,y)=2^r-c$ for any $c$.
Similarly to $EQ_g(x,y)$, we can also
define formulas $LT_g(x,y)$ to denote that its counter $C_g(x) < C_g(y)$,
$GT_g(x,y)$ to denote that $C_g(x) > C_g(y)$, etc.
Hence any form of threshold counting
relation can be replaced by an equisatisfiable formula, with
all these global counters running from the beginning of the word to the end.
Thus we have a polynomially sized equisatisfiable reduction from
\fotwothr\/ to \fotwobet.
\end{proof}

To complete the proof of Theorem~\ref{thm.fo2sat},
the upper bound for \fotwothr\/ comes from
Lemma \ref{lem.reduction}, an exponential translation
from \fotwobet\/ to \binvtl\/ using an order type argument similar to \cite{EVW}
(our Theorem~\ref{thm.tlequivalence} also points to this equivalence),
and the \pspace\/ upper bound for \binvtl\/ (Theorem~\ref{thm.utlsat}).
Again using standard order type arguments \cite{EVW}, we can translate
an $\fobetfac$ sentence to an exponentially sized \bfactl\/ formula,
whose satisfiability is decidable in \pspace\/ by Theorem~\ref{thm.utlsat}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "test.tex"
%%% End:

